A novel strong duality-based reformulation for trilevel infrastructure models in energy systems development

We explore the class of trilevel equilibrium problems with a focus on energy-environmental applications and present a novel single-level reformulation for such problems, based on strong duality. To the best of our knowledge, only one alternative single-level reformulation for trilevel problems exists. This reformulation uses a representation of the bottom-level solution set, whereas we propose a reformulation based on strong duality. Our novel reformulation is compared to this existing formulation, discussing both model sizes and computational performance. In particular, we apply this trilevel framework to a power market model, exploring the possibilities of an international policymaker in reducing emissions of the system. Using the proposed methods, we are able to obtain globally optimal solutions for a five-node case study representing the Nordic countries and assess the impact of a carbon tax on the electricity production portfolio.

==> macros.tex <==
\newcommand{\LPCC}{\text{LPCC}}
\newcommand{\LPCCx}{\text{LPCC}$(x)$}

\newcommand{\MS}[1]{\todo[author=MS,color=green!30]{\textsf{\small{#1}}}}
\newcommand{\ML}[1]{\todo[author=ML,color=orange!30]{\textsf{\small{#1}}}}
\newcommand{\SG}[1]{\todo[author=SG,color=blue!30]{\textsf{\small{#1}}}}
\newcommand{\MSil}[1]{\todo[author=MS,inline,color=green!30]{\textsf{\small{#1}}}}
\newcommand{\MLil}[1]{\todo[author=ML,inline,color=orange!30]{\textsf{\small{#1}}}}
\newcommand{\SGil}[1]{\todo[author=SG,inline,color=blue!30]{\textsf{\small{#1}}}}
\newcommand{\marina}[1]{{\color{orange}#1}}

\newcommand{\st}{\text{s.t.}}
\newcommand{\abbr}[1][abbrev]{#1.\xspace}
\newcommand{\abbrev}{\abbr}
\newcommand{\cf}{\abbr[cf]}
\newcommand{\eg}{\abbr[e.g]}
\newcommand{\etc}{\abbr[etc]}
\newcommand{\ie}{\abbr[i.e]}
\newcommand{\vs}{\abbr[vs]}
\newcommand{\wrt}{\abbr[w.r.t]}

\newcommand{\field}{\mathbb}
\newcommand{\naturals}{\field{N}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}

\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\defsep}{\colon}% alternative: \mid
\newcommand{\defset}[3][\defsep]{\set{#2#1#3}}
\newcommand{\Defset}[3][\defsep]{\Set{#2#1#3}}

\newcommand{\myeps}{\varepsilon}

\newcommand{\define}{\mathrel{{\mathop:}{=}}}
\newcommand{\enifed}{\mathrel{{=}{\mathop:}}}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\myforall}{\text{for all }}

% For the replies to the reviewers
\newcommand{\comment}[1]{\textbf{Comment: } \emph{#1}}
\newcommand{\reply}[1]{\textbf{Reply: } #1 \\}
\newcommand{\TODO}{\textcolor{red}{TODO }}

%\newcommand{\revDel}[1]{\textcolor{blue}{\sout{#1}}}
%\newcommand{\revNew}[1]{\textcolor{blue}{#1}}
\newcommand{\revDel}[1]{}
\newcommand{\revNew}[1]{#1}

\ifPreprint
\renewcommand{\cite}[1]{\textcite{#1}}
\fi

\ifJorsTemplate
\newcommand{\parencite}[1]{\cite{#1}}
\fi


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "bilevel-w-lower-level-lpcc-preprint"
%%% End:

